Adversarial Examples on Object Recognition: A Comprehensive Survey

Deep neural networks are at the forefront of machine learning research. However, despite achieving impressive performance on complex tasks, they can be very sensitive: Small perturbations of inputs can be sufficient to induce incorrect behavior. Such perturbations, called adversarial examples, are intentionally designed to test the network's sensitivity to distribution drifts. Given their surprisingly small size, a wide body of literature conjectures on their existence and how this phenomenon can be mitigated. In this article we discuss the impact of adversarial examples on security, safety, and robustness of neural networks. We start by introducing the hypotheses behind their existence, the methods used to construct or protect against them, and the capacity to transfer adversarial examples between different machine learning models. Altogether, the goal is to provide a comprehensive and self-contained survey of this growing field of research.

==> chapters/attacks/others/others_acm.tex <==
%\subsection{Other types of attacks}
%\label{subsec:others}
%
%% TODO: Decide on this sentence
%% In this section we explore peculiar attacks - which do not fit any of the classes presented before.
%
%Although most publications consider adversarial examples in close resemblance to inputs drawn from the training set, the authors of~\cite{nguyen2015deep}
%	craft special images that can not be understood by human observers, but can generate a targeted classification with over $90\%$ accuracy.
%The authors leverage evolutionary algorithms~\cite{cullyrobots} in order to evolve candidate solutions that can fool \ac{DNN}.
%The fitness function evaluates candidates by sending the image to a target \ac{DNN}.
%
%Instead of using gradient based optimisation techniques in order to change only one pixel of an image, the authors of~\cite{su2017one} use differential evolution~\cite{storn1997differential} - an evolutionary optimisation method that ensures high population diversity.
%In order to define a fitness function, only the output of the softmax function is required.
%For targeted attacks, the fitness function aims to increase the probability of a target class; while for un-targeted attacks it aims to decrease the probability of the true class.
%While it requires less information about the model under attack, this attack performs poorly when compared to gradient-based methods.

\if 0\mode \bigskip \else  \newpara  \fi

\subsection{Attacks using Adversarial Examples on other \ac{ML} Tasks}
\label{subsec:real_world}

Attacks using adversarial example were explored for other tasks than object recognition.
Of particular interest is the task of malware detection~\cite{grosse2016adversarial, hu2017generating, laskov2014practical, xu2016automatically, kreuk2018adversarial} because it poses high security risks.
Other tasks explored come from the fields of reinforcement learning~\cite{behzadan2017vulnerability, huang2017adversarial, lin2017tactics},
speech recognition~\cite{carlini2016hidden, carlini2018audio}, facial recognition~\cite{sharif2016accessorize}, semantic segmentation~\cite{xie2017adversarial} or video processing~\cite{wei2018transferable, li2018adversarial}.
%However, none of these publications present an accurate threat model or judge the economics of carrying an attack using adversarial examples, in comparison to other attack methods.
Other publications explore the impact of adversarial examples in the physical world - by printing corrupted images~\cite{evtimov2017robust, kurakin2016adversarial} or altering the image acquisition device (\eg~phone camera, digital camera, \etc)~\cite{moosavi2017universal}.


It seems that adversarial examples can be found for most tasks where \ac{ML} algorithms are used.
However, their true impact on safety or security is hard to evaluate without developing appropriate threat models specific to each task.
We touch upon this subject in Section~\ref{sec:discussion}.

==> chapters/defences/obfuscate/obfuscate.tex <==
% TODO: talk about transferability between differentiable and non-differentiable models !!!

\subsection{Obfuscated Defences}
\label{subsec:obfuscated_defences}

%\input{chapters/defences/obfuscated}


==> chapters/defences/obfuscated.tex <==
%\subsection{Obfuscated Gradients}
%\cite{athalye2018obfuscated}

%The authors of~\cite{athalye2018obfuscated} identify another reason why many defences provide apparent robustn
%Another reason for which defences provide apparent robustness against powerful, iterative, attacks is called \emph{obfuscated gradients}~\cite{athalye2018obfuscated} - a term derived as a special case of gradient masking~\cite{papernot2017practical}.
%Without a good gradient, iterative methods can not follow succeed.
%These phenomena occurs when the gradients are nonexistent or incorrect - caused either intentionally through non-differentiable operations or unintentionally through numerical instability - when the gradient is unstable - due to vanishing/exploding gradients - or randomly due to test-time randomness.


==> chapters/defences/proactive/adversarial_training/training_vs_weight_decay.tex <==
\subsection{Advers}
\label{subsec:training_vs_decay}
% TOOD: label leaking

The first attempt to scale adversarial training to ImageNet~\cite{kurakin2016aadversarial} revealed an interesting phenomena, called 'label leaking' - when a network is trained with adversarial examples, the accuracy on adversarial examples becomes much higher that the accuracy on clean images.
This phenomena triggered the authors of~\cite{galloway2018adversarial} to compare the effects of adversarial training with weight decay - a regularisation technique understood mathematically.
The results suggest that adversarial training can be seen as translating the data \ac{wrt} the loss function, while weight decat scales the let-on-(about-sth/that...)-(to-sb)




==> chapters/defences/proactive/adversarial_training/virtual.tex <==
\subsubsection*{Virtual Adversarial Training}
\label{subsubsec:virtual}

%Towards Safe Deep Learning: Unsupervised Defense Against Generic Adversarial Attacks

==> chapters/defences/proactive/architectures/logit_pairing.tex <==
\subsection{\ac{alp}}
\label{subsuec:logit_pairing}

\ac{alp}~\cite{kannan2018adversarial} is a method that encourages the logits for two images to be similar to each other.
Logit pairing adds a loss penalty $\lambda L(f(\vx), f(\vx')$ for pairs of training examples $\vx$ and $\vx'$, where $\lambda$ is a coefficient that regulates the strength of the penalty and $L$ is a loss function encouraging the logits to be similar.
In practice, the authors use $L^2$ loss.
The method is similar to label smoothing~\cite{szegedy2016rethinking}, a technique showed to offer a small amount of robustness to adversarial examples~\cite{warde201611}.

Logit pairing achieves high accuracy against the attack in Section~\ref{subsec:madry}, considered, at this time, state-of-the art.
Moreover, attacks built on networks trained with \ac{alp} substantially damage black box defences~\cite{tramer2017ensemble}.


==> chapters/defences/proactive/g <==
\subsubsection{\ac{mat}}
\label{subsubsec:multi_strength_training}

Song \etal~\cite{song2017mat} propose a training technique that combines several aplitude of pertubations in the training procedure.
The technique is equivalent to an ensemble of perturbations (Section~\ref{subsec:ensemble}), however training does not happen in a min-max fashion.

Experimental results show improvements in robustness, however, it is not clear if this method is effective when faced with adaptive attacks.



==> chapters/defences/proactive/gans/gradient_adversarial_training.tex <==
\subsubsection{Gradient Adversarial Training}
\label{subsubsec:gradient_adversarial}

Sinha \etal~\cite{sinha2018gradient} propose a new training framework which assumes that simultaneous gradient updates should be statistically indistinguishable from each other.
% TODO: Why? Mention Adversarial
Thus the gradient can be regularised in order to remove salient information that can lead to adversarial examples.
This phenomena, called gradient obfuscation, is described in Section~\ref{}. % TODO: add section on gradient obfuscation
Further on, the gradient tensor is processed in an auxiliary network and then passed to the main network via a gradient reversal procedure.
This training procedure adapts the cross-entropy loss function and adds weight to negative classes whose gradient tensors are similar to those of the primary class.
The weight weight is evaluated using the auxiliary network which indicates the gradient tensors similarities between the primary and negative classes.

Experimental results show better regularisation during training and an increase in robustness when tested against gradient adversarial attacks.
However, robustness is not always preserved when testing is done agaist iterative gradient methods (Section~\ref{subsec:illcm}).



==> chapters/defences/proactive/gans/multi_strength_training.tex <==
\subsubsection{\ac{mat}}
\label{subsubsec:multi_strength_training}

Song \etal~\cite{song2017mat} propose a training technique that combines several aplitude of pertubations in the training procedure.
The technique is equivalent to an ensemble of perturbations (Section~\ref{subsec:ensemble}), however training does not happen in a min-max fashion.

Experimental results show improvements in robustness, however, it is not clear if this method is effective when faced with adaptive attacks.



==> chapters/defences/reactive/detection/detection_efficiency.tex <==
\subsection{On The Overall Efficiency of Detection Methods}
\label{subsubsec:detection_efficiency}


% TODO: review all
\input{chapters/defences/reactive/detection/detection_efficiency}
\input{chapters/defences/reactive/input_transformation/input_transformation_remarks}




An important disadvantage of all the papers presented earlier is their evaluation method.
Because they are tested on simple data sets (such as MNIST~\cite{lecun1998mnist}) or against non adaptive attackers, the results presented in the publications reveal fairly good performance for all detectors.
However, Carlini and Wagner~\cite{carlini2017adversarial} show most detectors perform poorly when faced with an adaptive attacker.
In particular, they use the attack presented in Section~\ref{subsec:carlini} to show that none of the detectors -\cite{bhagoji2018enhancing, feinman2017detecting, gong2017adversarial, grosse2017statistical, hendrycks2016early, metzen2017detecting, li2017adversarial} - are efficient against it.

These results challenge the assumption made at the beginning of this section that adversarial examples have intrinsic differences from natural images.

%% TODO: say neither of those are tested against adaptive attacks!!!

==> chapters/defences/reactive/input_transformation/input_transformation_remarks.tex <==
\subsubsection{Remarks Regarding Input Transformation}
% They do not generalise, so one input transformation should be applied to a specific architecture, which makes such techniques hard to apply

==> chapters/distilled/distilled_acm.tex <==
\section{Conclusions}
\label{sec:conclusions}
% \paragraph{Conclusions}
\label{sec:conclusions}
We focused on several points related to the adversarial examples phenomenon.
In this section, we summarise and comment on the key ideas underpining this research field.

% \subsection{Discussion}
\paragraph{Short Summary and Discussion.}
\label{subsec:discussion}

As mentioned in Section~\ref{sec:causes}, an unanimously accepted conjecture on the existence of adversarial examples is still missing.
Overall, we can distinguish between two lines of thought: (1) adversarial examples are drawn from the same data distribution as normal inputs and lie on the same data manifold, therefore, their existence is due to selecting a bad hypothesis from the hypothesis space or due to a small training data set, and (2) adversarial examples are part of a different data distribution and lie off the data manifold.
At the moment of writing this survey there is not enough theoretical or empirical data to refute any of these conjectures.
Threfore, this perspective leaves room for a lot of research questions.

Moreover, the literature offers many definitions of robustness (as outlined in Section~\ref{sec:robustness_eval}).
Most methods focus on the area around an input where no adversarial examples can be found or on the maximum size of a perturbation that can be applied to an input in order to generate adversarial examples.
Because the focus is on particular inputs, it is not yet clear how these definitions generalise to the whole data manifold.

In practice, most publications resume to computing the expectation of the error when the \ac{ML} model is tested against adversarial examples.
Therefore, the evaluation method depends heavily on the underlying \ac{ML} model and the data set used, making it difficult to compare defences.
We concluded Section~\ref{subsec:overall_defences} with a short protocol for future evaluation of \ac{ML} models against adversarial examples; which should consider large networks and data sets.

The phenomenon of adversarial examples is thought to have an impact on the security of \ac{ML} models.
It is true that various attacks could, in principle, be carried using adversarial examples.
However, it is not always clear \emph{why} an attacker would prefer to use adversarial examples instead of other methods of achieveing the same goal.
Without considering the economics of using adversarial examples and defining clear threat models, the security implications of adversarial examples remain fuzzy.
In order to help shape future research in this direction, we dedicate a section (Section~\ref{sec:attack_models}) to threat modeling and discuss the security implications of adversarial examples in real world scenarios.
% In order to ease ... we present, etc.  mention section on attack capabilities!

At the moment, most research concerning adversarial examples focuses on finding a perturbation that is minimal or, at least, indistinguishable by human observers.
Although the existence of such small perturbations is an important property, research should not be limited by it, since in practical scenarios machines will not be supervised by humans.
A uninanimous decision for when the sensitivity to adversarial examples is removed (\ie when the problem is solved) is still lacking.
In many cases, this decision can be context-dependent (as suggested in Section~\ref{sec:robustness_eval}) however, several research directions can be traced  based on this decision.

Because the research in adversarial examples is still young, it is not yet clear which is the impact this phenomenon will have on the overall research in \ac{DL}.
Do adversarial examples reveal a more deep phenomenon, \eg~that \ac{DNN} learn differently than humans do?
If so, are there some lessons we can learn in order to develop better computer vision (and other) algorithms?
We discuss some of these questions in future research.

% \subsection{Contributions}
\paragraph{Summary of Contributions.}
\label{subsec:contributions}
Our contributions are manyfold, and can be summarised as follows:

\begin{itemize}
    \item We provide a synthesis of this research field that is not only concerned with attacks and defences, but also takes into account \emph{threat modeling} and the \emph{safety, security} and \emph{robustness} implications (and definitions).
    \item We provide an in-depth analysis of the hypotheses on the existence of adversarial examples.
    \item We treat in details the phenomenon of transferability of adversarial examples between different \ac{ML} models.
    \item We shape a taxonomy for the attacks and defences techniques presented in the literature.
    \item We provide an exhaustive list of attacks and defences.
    \item We present interesting directions for future research.
\end{itemize}


% \subsection{Directions for Future Work}
\paragraph{Directions for Future Research.}
\label{subsec:future_work}

The short summary and discussion presented earlier in this section leads to the following research directions:

\begin{itemize}
    \item Fundamental analysis of the existence of adversarial examples. Since the causes of adversarial examples are not known, more fundamental research concerning this phenomenon is needed. Some interesting research directions can spark from a geometric analysis of the data manifold and of the decision boundaries, an investigation concerning the number of samples needed (similar to PAC-learning) or concerning general resources needed for robust models (\eg~computation power).
    \item New ways to define robustness.
    \item New methods to define and evaluate when the phenomenon is (completely) removed.
    \item New defence mechanisms which should reflect the robustness definitions mentioned earlier.
    \item New (and faster) methods to approximate uncertainty sets around an input, which will lead to better adversarial training.
    \item New (faster and scalable) methods to certify robustness.
    \item New types of attacks and threat models using adversarial examples.
\end{itemize}

%% approximate the uncertainty sets better

==> chapters/taxonomy/old_taxonomy.tex <==
\section{Taxonomy and Threat Modeling}
\label{sec:taxonomy}

The literature concerning adversarial examples focuses on the security consequence they imply.
Nonetheless, their real impact on security has been a subject of debate; with some publications claiming a severe impact and others being more skeptical~\cite{oneval, gilmer2018motivating}.
Nevertheless, since security aspects are prevalent in literature, we discuss, at first, adversarial examples from this perspective.

In order to analyze the security of a system, one needs to identify security goals and threat models~\cite{barreno2010security}.
Security goals are requirements specifying which assets have to be protected from attackers, while threat models represent the attacker's profile, their knowledge and capabilities.
% CIA
Information security is governed by three goals: protecting the information (1) Confidentiality, (2) Integrity and (3) Availability (CIA).
In the first case, the  goal is to forbid attackers from extracting information about the model or the training data.
By protecting integrity, the system denies the attackers access to system assets and forbids behavior induced by an attacker.
Protecting availability forbids attackers from interfering with the normal operation of a system and ensures users have access to the system at any time.

The CIA framework is used in the early taxonomies~\cite{barreno2006can, barreno2010security} and later modified in~\cite{papernot2016towards}, when \citeauthor{papernot2016towards} consider availability and integrity as one goal.
We note that an attacker can mount an attack against a \ac{ML} system at either training or inference time.
From this perspective, adversarial examples represent a threat only to the \emph{integrity} of \ac{ML} algorithms at \emph{inference} time; defined as exploratory attacks in the early taxonomies~\cite{barreno2006can, barreno2010security}.

In general, security is modeled as a game between two players: an attacker and a defender, with each making a series of moves or steps~\cite{barreno2010security}.
For example, the attacker chooses a range of perturbations she wants to apply and the defender chooses a training procedure.
We use this setting, together with early taxonomies to sketch the profile of the attacker and the defender.

\subsection{Attacker}
\label{sec:taxonomy_attacks}
The attacker's profile is also called a threat model.
In literature, there are three proposed dimensions for threat modeling, taking into account (1) the attacker's goal, (2) the attacker's knowledge and (3) the attacker's capabilities~\cite{barreno2010security, biggio2017wild, papernot2016limitations}.
However, the definitions do not always concur.
\citeauthor{barreno2010security} define the attacker's goals as generating false negatives or false positives~\cite{barreno2010security}.
\citeauthor{biggio2017wild} describe the attacker's goal using two dimensions: the \emph{attack specificity}~--~if an attacker causes a misclassification for a set of samples or for any sample~--~and the \emph{error specificity}~--~if an attacker aims to misclassify a sample as a specific class or not~\cite{biggio2017wild}.
\citeauthor{papernot2016limitations}~\cite{papernot2016towards} and \citeauthor{oneval}~\cite{oneval}, targeting only attacks with adversarial examples on \acp{DNN}, describe the attacker's goal using only the error specificity introduced by \citeauthor{biggio2017wild}~\cite{biggio2017wild}; since in this particular  case, the attack specificity refers to misclassifying one sample.

Regarding the attacker's capabilities, \citeauthor{barreno2010security}~\cite{barreno2010security} and \citeauthor{biggio2017wild}~\cite{biggio2017wild} use the influence an attacker has on the training data to define two capabilities: (1) the ability to modify or generate data used in training (causative attacks) or (2) the ability to modify or generate samples used for inference (exploratory attack).
In contrast, \citeauthor{papernot2016limitations}~\cite{papernot2016limitations} define the attacker capabilities in terms of the knowledge she has about the model under attack.
Later, \citeauthor{oneval}~\cite{oneval} define the attacker's capabilities using the distance functions defined in Section~\ref{sec:background}, while maintaining a separate description of the attacker's knowledge.

In this paper, we follow the initial definition from \citeauthor{barreno2010security}~\cite{barreno2010security}, in which the attacker's capability is discussed \wrt~the influence she has on the training data.
Following this classification, adversarial examples belong to the second class, in which an attacker does not have the ability to modify the training data and can only control the samples used for inference.
This choice was made in order to preserve the attacker's knowledge as a distinct dimension.
Moreover, the definition from~\citeauthor{oneval}~\cite{oneval} only applies to publications which use the p-norm distance function (which is the most significant body of literature, but not the only one).

Further on, we discuss one extra dimension specific only to adversarial examples, meant to capture the large array of techniques used to generate them~--~called the \emph{attack strategy}.
The attack strategy characterizes the methods and the data used by an attacker to achieve a goal.
The strategies presented are extracted from the attacks discussed in Section~\ref{sec:attacks}.
Each dimension is discussed in detail in the following sections.


% TODO: discuss this a bit more these choices - say why there are important - because they describe the different possible ways in which adversarial examples can be generated, ranging from Gaussian noise to making small geometrical changes to known inputs.
% tells us / evidentiates how diverse this field is
% it allows us to extract higher level information about neural networks - discussed in a discussion section - e.g. their linear behaviour, the fact that the decision manifold is so intricate, the geometry of the decision boundaries and so on.
% although optimization is a higher level view, the diversity of algorithms applied, in different settings is impressive



\subsection*{Attacker Goal}
Attackers using adversarial examples aim to modify or generate one input, forcing a \ac{ML} system to produce an erroneous output.
Therefore, the attack specificity described by \citeauthor{biggio2017wild}~is always targeted~\cite{biggio2017wild}.
Similar to \citeauthor{papernot2016limitations}~\cite{papernot2016limitations}, we define the attacker's goal in terms of the error specificity \ie~if the attacker aims to have a sample misclassified as a random or a specific class.
The latter case has been referred to as a targeted attack~\cite{carlini2017towards}, a source-target attack~\cite{papernot2016limitations} or a specific error~\cite{biggio2017wild}.
In this paper, we use the term \emph{targeted attack}, as in~\citeauthor{carlini2017towards}~\cite{carlini2017towards}, and drop the dimension specific to the input data; unlike \citeauthor{papernot2016limitations}~\cite{papernot2016limitations} which make a difference between targeted and source-targeted misclassifications.
This choice was made in order to preserve a distinction between the attacker's goal and the data used.
We find that an attacker will first establish a goal and only afterwards search for the data needed to fulfill it.
Moreover, the input data are inherent to the attack strategy.

Depending on a specific use-case, an attacker can mount an:
\begin{itemize}
	\item \emph{Untargeted attack.} In this case an attacker designs an adversarial example in order to output \emph{any class} different than the correct one.
	\item \emph{Targeted attack.} In this case an attacker designs an adversarial example in order to output a \emph{specific, target, class}.
\end{itemize}



\subsection*{Attacker Knowledge}

Attackers can have different knowledge of the system under attack, related to the training data, the learning algorithm, the loss function or the hyper-parameters used.
In some cases, when the development of \ac{ML} models is tightly coupled with powerful hardware, the capability of an attacker can be limited by her inability to train large models.
However, we exclude this restriction and only consider attackers unbounded by hardware constraints.
Depending on the attacker's knowledge, one can identify two scenarios:

%
\begin{itemize}
	\item \emph{White box.} The adversary has complete knowledge of the model, its parameters or the data and can completely replicate the model under attack.
%	\item \emph{Grey box.} The adversary has partial knowledge about the model, the data or any defenses employed for protecting against adversarial examples but the information is neither complete or certain so the attacker can only partially replicate the model under attack.
	\item \emph{Black box.} The adversary has no knowledge of the model or the data used in training and can not replicate the model. In this case, one can make different assumptions about the attacker's ability to query the model indefinitely or limited, to access the output probability distribution or just one class, \etc
\end{itemize}
\noindent
This classification corresponds to the one adopted in~\cite{papernot2016limitations, papernot2016towards}.
\citeauthor{biggio2017wild}~\cite{biggio2017wild} also consider the grey-box scenario, in which an attacker has only partial knowledge about the model.
However, this scenario is not common in the adversarial examples literature and it is often seen as a special case of the black box scenario, in which the attacker is more restricted (\eg~by the number of queries sent to the oracle)~\cite{oneval}.

An attacker might also have access to pairs of inputs and outputs collected from a classifier, but no ability to modify the inputs or test them with an oracle.
This scenario can help to extract some information about the model, by reverse-engineering the data, however it is not explored in the field of adversarial examples.

\subsection*{Attack Strategy}
The term attack strategy has been introduced by \citeauthor{biggio2017wild}~\cite{biggio2017wild} to describe the method used by an attacker to achieve a goal (given its knowledge) and select the optimal method.
In this paper we do not use the attack strategy in the optimal way envisioned by \citeauthor{biggio2017wild}~\cite{biggio2017wild}.
Instead, we define the attack strategy as the method used to generate adversarial examples, given the attacker's goal and knowledge about the system under attack~--~since the attack optimality in relation to the attacker goal is rarely discussed in the literature.

Although most algorithms for finding adversarial examples rely on optimization constructs, we distinguish between algorithms that use optimization methods to find solutions to \eqq~(\ref{eq:adversarial_generic}) and algorithms that use optimization methods as a mean to achieve other goals, such as discovering sensitive features.
Overall, we identify four attack strategies:

\begin{itemize}
	\item \emph{Optimization Strategy.} Attackers applying this strategy use optimization algorithms to search for solutions to \eqq~(\ref{eq:adversarial_generic}) or alternative forms. In some cases, the solutions are exact, resulting in strong and precise attacks, with the cost of increased processing time.
	\item \emph{Sensitivity Analysis.} This attack strategy finds and perturbs sensitive features in order to cause a misclassification. For example, one can find a small set of pixels from an image that can be perturbed in order to induce a classification error. It is often the case that sensitivity analysis requires optimization techniques~\cite{yeung2010sensitivity}, however, these are only used to discover the features to be perturbed and not the perturbation.
	\item \emph{Geometric Transformations.} Perturbations based on noise are not the only way to create adversarial examples. More natural, geometric transformations (such as rotations or translations) have also been used to generate adversarial examples are though to appear more frequently in normal operational environments~\cite{engstrom2017rotation}.
	\item \emph{Generative Models.} The strategies mentioned above rely on accessing and modifying a sample from the data generation distribution. Whenever such a sample is not available, the attacker has to generate one. This attack strategy captures the techniques used to generate an adversarial example from scratch.
\end{itemize}

The attack taxonomy can be visualized in Table~\ref{tbl:attacks}, together with the quality attributes specific to each attack (discussed later, in Section~\ref{sec:attacks}).
We observe that most attacks assume full knowledge of the model and make use of sensitivity analysis.
This is due to the fact that attacks using the optimization strategy are, in general, slower, limiting their utility in other contexts such as training a model with adversarial examples.
Therefore, they are not explored to a great extent and are mainly used to bring evidence for different conjectures.
Nevertheless, the impact of the optimization strategy is significantly higher for black box attacks.

Contrary to the optimization strategy, the sensitivity analysis strategy is (generally) faster, although it always requires full knowledge of the model under attack.
An exception is observed when the attacker wants to transfer adversarial examples from a white box to a black box setting.
In this case, the attacker has to first train a white box model for crafting adversarial examples, then transfers them to an unknown model.

We observe that no attacks based on geometric transformations or generative strategies are mounted in a black box settings.
In the case of generative models, an approximation of the data generation distribution is needed.
However, one might try to train a substitute generative model and transfer the adversarial examples, as in the case of black box sensitivity attacks.
Moreover, some attacks based on geometric transformations can be mounted without changes in black box settings.

\input{chapters/attacks/acm_table}





\subsection{Defender}
\label{sec:taxonomy_defense}
As mentioned earlier, security is modeled as a game between an attacker and a defender, in which each participant makes a series of steps.
The defender can either improve the system \emph{in response} to new adversarial threats or \emph{anticipate} threats and design the system with security in mind.
In the first case, the defender is said to be \emph{reactive}.
One disadvantage of reactive security is that it can only protect against known threats.
Whenever the defender anticipates adversarial threats and designs systems capable of withstanding them, the defender is said to be \emph{proactive}.

This taxonomy has been used for \ac{ML} security~\cite{biggio2012poisoning, liu2018survey}, however, the field of adversarial examples has been mainly focusing on defenses against perturbations in the p-norm ball around one input.
Since this threat is already known, one can state that the vast amount of literature on this topic focused on reactive defenses, given that a scalable and flexible solution to this problem is not yet available~\cite{oneval}.

Therefore, we model the defender only in terms of her defense strategy, similar to the attack strategy presented in Section~\ref{sec:taxonomy_attacks}.
This classification is meant to give an overview of the vast and dissimilar work that has been done on this topic.
It is worth mentioning that protecting against perturbations in the p-norm ball is not the solely requirement to guarantee security, as argued in a series of publications~\cite{gilmer2018motivating, oneval, papernot2018marauder}.
This topic is discussed in Section~\ref{sec:discussion}.

\subsection*{Defense Strategy}
\label{subsec:defense}
Similar to the attack strategy, we define the defense strategy as the method used to defend against adversarial examples.
At a high level of abstraction, defense strategies can be classified using the step in the processing pipeline where they act.
Some defense strategies act early in the processing pipeline, before an input reaches the \ac{ML} model, while others are meant to strengthen the model directly.
We call the first class of defenses \emph{guards}, because they do not interact with the model under attack, but only try to protect the model building precautions around it.
The second class of defenses acts directly on the model, by modifying its architecture, the training data or the loss function.
We refer to such defenses as \emph{defenses by design}, since they employ a direct change of the model.


We further decompose the two classes of defense strategies based on the methods used, in:
\begin{itemize}
	\item \emph{Guards.}
		\begin{itemize}
			\item \emph{Detection.} Adversarial detection methods assume that adversarial examples have special characteristics or are sampled from a different data distributions than normal inputs. Therefore, it was hypothesized that a detector can learn to identify adversarial examples.
			\item \emph{Input Transformation.} Defenses in this class use pre-processing techniques such as compression or bit-depth reduction in order to remove the effect of adversarial perturbations and their impact on the model under attack.
		\end{itemize}
	\item \emph{Defense by Design.}
	\begin{itemize}
		\item \emph{Adversarial Training.} Given that learning is a data driven process, a normal defense strategy is to include adversarial examples in the training process.
		\item \emph{Architectural Defenses.} Another strategy is to design new architectures and models with constraints related to adversarial examples, such as custom regularization.
		\item \emph{Certified Defenses.} An interesting approach to defending against adversarial examples is to formally certify that within some bounds no adversarial examples can be found. Although this strategy sometimes overlaps with architectural defenses (since most certified defenses require new designs) the goal of these defenses is different. Therefore, they are specified in a different category.
	\end{itemize}
\end{itemize}

The defense taxonomy is illustrated in Table~\ref{tbl:defences_acm}, together with quality attributes specific to each defense (discussed later, in Section~\ref{sec:defences}).
Guards are of interest because they do not impose restrictions on the \ac{ML} model under attack.
While training adversarial detectors requires more resources and might also suffer from lack of robustness, input transformations aim to reduce the space where adversarial perturbations lie and do not require high computational resources.
Such attributes are important because they make defenses easy to implement and adopt.

Since \ac{ML} is a data driven process, a normal reaction to adversarial examples is to include them in the training set.
This method, called adversarial training, is a way of regularizing the model for increased robustness and shows good results when the space of the perturbations can be well approximated.
Moreover, adversarial training provides benefits for the model, such as more interpretable gradients~\cite{tsipras2018there}.
% However, while some methods for adversarial training provide state-of-the-art defenses~\cite{madry2017towards}, they are far from optimal.

In an analogous manner, architectural defenses rely on imposing regularization penalties. This time, however, the constraints are applied layer-wise, to the input data or to the final layer.
These constraints go beyond enhancing the training data set with adversarial examples and require new architectural designs or constraints.
% While interesting in nature, architectural defenses do not offer increased robustness when compared to adversarial training or certified defenses.

Until now, the defense strategies introduced can not \emph{guarantee} robustness and only rely on approximations.
Contrary, certified defenses can guarantee that no adversarial examples can be found within some bounds.
These defenses show great potential for both finding spots where \acp{DNN} fail and for improving them.
However, certified defenses are not yet scalable to deep models and often require high computational resources.


% TODO: comment on the number!
\input{chapters/defences/table_acm}

